CryptMPI: A Fast Encrypted MPI Library

The cloud infrastructure must provide security for High-Performance Computing (HPC) applications of sensitive data to execute in such an environment. However, supporting security in the communication infrastructure of today's public cloud is challenging, because current networks for data centers are so fast that adding encryption can incur very significant overheads. In this work, we introduce CryptMPI, a high performance encrypted MPI library that supports communication with both integrity and privacy. We present the techniques in CryptMPI and report our benchmarking results using micro-benchmarks and NAS parallel benchmarks. The evaluation results indicate that the aforementioned techniques are effective in improving the performance of encrypted communication.

==> analysis.tex <==

\section{Modeling Encrypted Ping Pong}

To understand the individual contribution of Chopping and Multi-threading Encryption,  
we model the performance of encrypted Ping Pong when (i) only Chopping is used, and (ii) only Multi-threading Encryption is used. 
We then model the interaction of Chopping and Multi-threading Encryption in  CryptMPI's Ping Pong. 
In our models, we assume that a sender can concurrently transmit the ciphertext of a message via a non-blocking send
and encrypt the next message. A receiver likewise can decrypt the current ciphertext while getting the next ciphertext via a non-blocking receive.


\heading{The Hockney model.}

\heading{Modeling Encryption-Decryption.}





\subsection{Ping Pong with Chopping}


\noskipheading{Model description.}
Suppose that we chop a message of~$m$ bytes into $s$-byte segments. 
For simplicity, assume that $m$ is a multiple of $s$. 
As the ciphertext segments are sent successively, the latency term $\acomm$ is only 
manifest in the transmission of the last ciphertext segment. 
Since the encryption of each $i$-th segment can overlap with the transmission of the 
ciphertext of the $(i - 1)$-th  segment  for every $i \in \{ 2, \ldots, m / s\}$, 
the time to encrypt and transmit the entire message is 
\[ 
\frac{\Ted(s)}{2} + \Bigl( \frac{m}{s} - 1\Bigr) \max\Bigl\{ \frac{\Ted(s)}{2} , \bcomm \cdot s \Bigr\} + \Tcomm(s) \enspace. 
\] 
During this time, the receiver can decrypt all but the last ciphertext, 
 and thus it will need $\frac{\Ted(s)}{2}$ additional time units to decrypt the last ciphertext. 
Hence the total time is
\[ 
\Ted(s) + \Bigl( \frac{m}{s} - 1\Bigr) \max\Bigl\{ \frac{\Ted(s)}{2} , \bcomm \cdot s \Bigr\} + \Tcomm(s) \enspace. 
\] 

\noskipheading{Discussion.}

\heading{Model validation.}


\subsection{Ping Pong with Multi-threading Encryption}

\noskipheading{Model description.}
Suppose that we use $t$ threads to encrypt a message of~$m$ bytes. 
Assume that $m$ is a multiple of $t$. 
Then the total time to encrypt~$t$ segments, transmit them, and then decrypt them is about
\[
\Ted(t, m / t) + \Tcomm(m) \enspace. 
\] 
If $t = 1$ then we get back the model of Naser et al.~\cite{Cluster:Naser19} for their vanilla implementation of encrypted Ping Pong. 

\heading{Model validation.}


\subsection{Ping Pong under CryptMPI}

\noskipheading{Model description.} Suppose that we chop a message into $s$-byte segments, 
and use $t$ threads to encrypt each segment. Assume that $m$ is a multiple of $s$, and $s$ is a multiple of $t$.  
We model the latency of encrypted Ping Pong as
\[ 
\Ted(t, s / t) + \Bigl( \frac{m}{s} - 1\Bigr) \max\Bigl\{ \frac{\Ted(t, s/t)}{2} , \bcomm \cdot s \Bigr\} + \Tcomm(s).
\] 
This is essentially the model of Chopping's Ping Pong, where each $\Ted(s)$ is replaced by $\Ted(t, s/t)$. 

\heading{Discussion.}

\heading{Model validation.}

\iffalse

\subsection{Privacy Analysis} 


In our privacy threat model, an adversary passively collects network packets sent
from the MPI nodes and tries to infer partial information about the MPI program and input.\footnote{We assume that the MPI program does not have MPI\_Reduce or MPI\_Allreduce, 
since $\sysrm$ currently does not support these two routines.}
The adversary, however, does not have physical access to the machines. 
This restriction eliminates side-channel attacks such as the rowhammer attack~\cite{rowhammer}.
Thanks to the semantic security of encryption~\cite{GM84,BDJR97}, 
the adversary cannot distinguish a ciphertext segment and a uniformly random string of the same length. 
Despite encryption, the adversary still gets some \emph{metadata} 
of the program and input: the message length,  the routine type
(Send, Broadcast, Scatter, or AlltoAll), and the execution timings. 
$\sysrm$ guarantees that the adversary does not learn anything beyond
what can be inferred from the metadata and the adversary's prior knowledge of the MPI program and input. 





\subsection{Authenticity Analysis}

In our authenticity threat model, an adversary first requests the execution of an adversarial MPI program and input, 
and then actively tries to modify the ciphertext segments 
in the network packets without detection. 
The adversary is, however, not allowed to launch a \emph{replay attack}, 
that is, it is forbidden from replacing the entire vector of ciphertext segments
$(C_1, \ldots, C_m)$ of $\vecM = (M_1, \ldots, M_m)$
by the entire vector of ciphertext segments of a prior message.\footnote{
This restriction is due to the fact that GCM is deterministic: 
under the same key and nonce, encrypting the same message via GCM multiple times
will always result in the same ciphertext.}
The authenticity of $\sysrm$ (assuming that Chopping GCM is used) follows directly from the authenticity of Chopping GCM. 
We stress that $\sysrm$ with $\FastCTR$ offers no authenticity. 

\fi
